Economical routes to size-specific assembly of self-closing structures

Self-assembly is one of the prevalent strategies used by living systems to fabricate ensembles of precision nanometer-scale structures and devices. The push for analogous approaches to create synthetic nanomaterials has led to the development of a large class of programmable crystalline structures. However, many applications require `self-limiting' assemblies, which autonomously terminate growth at a well-defined size and geometry. For example, curved architectures such as tubules, vesicles, or capsids can be designed to self-close at a particular size, symmetry, and topology. But developing synthetic strategies for self-closing assembly has been challenging, in part because such structures are prone to polymorphism that arises from thermal fluctuations of their local curvature, a problem that worsens with increased target size. Here we demonstrate a strategy to eliminate this source of polymorphism in self-closing assembly of tubules by increasing the assembly complexity. In the limit of single-component assembly, we find that thermal fluctuations allow the system to assemble nearby, off-target structures with varying widths, helicities, and chirality. By increasing the number of distinct components, we reduce the density of off-target states, thereby increasing the selectivity of a user-specified target structure to nearly 100%. We further show that by reducing the design constraints by targeting either the pitch or the width of tubules, fewer components are needed to reach complete selectivity. Combining experiments with theory, our results reveal an economical limit, which determines the minimum number of components that are required to create arbitrary assembly sizes with full selectivity. In the future, this approach could be extended to more complex self-limited structures, such as shells or triply periodic surfaces.

==> MonomerSequence-10_0.tex <==
Name & Sequence \\
\hline
\endfirsthead

Name & Sequence \\
\hline
\endhead

\endfoot
\endlastfoot
(10,0) Side 1 Position 1	&	ACGTATAAAAATCGGAACCCTAAATTXXXXXX	\\			
(10,0) Side 1 Position 2	&	TCGCCATGAGAATATAAAGATGACAGGGAATTXXXXXX	\\			
(10,0) Side 1 Position 3	&	AGAGATAGAACCCTTCCACTTTTGGGGTCGAGTTXXXXXX	\\			
(10,0) Side 1 Position 4	&	TACCATTAGCAAGGCCATAATAAGAGCGCTAATTXXXXXX	\\			
(10,0) Side 1 Position 5	&	GCGTTTGCCATCTTTGTTTTCACCTTTAGTGGTAATCAGATGCTTXX	\\	&	XXXX	\\
(10,0) Side 1 Position 6	&	CGCAGTATGTTAGCAATTAAGACTTAGCTATCACTGGTGTTTXXXXX	\\	&	X	\\
(10,0) Side 2 Position 1	&	CCTTATAAAAGGAAACCGAGGCCCGGTCACTGTTXXXXXX	\\			
(10,0) Side 2 Position 2	&	GATTAGCATAGCCCGGAATAAATTTTTCATTTXXXXXX	\\			
(10,0) Side 2 Position 3	&	TTTCACCAGTGAGACGACACACTCAATCCGCCTTXXXXXX	\\			
(10,0) Side 2 Position 4	&	CACGGCCCGACCGCATACCAGTCAGGACGCCCCCAGCCTAAAACGTT	\\	&	XXXXXX	\\
(10,0) Side 2 Position 5	&	GAATTACGAGGCATAACCACATTTCATCAAGACTTCCTCCGTGTTXX	\\	&	XXXX	\\
(10,0) Side 2 Position 6	&	TCAATTTTCATAAGGGAACCGAACTGTACAACGTAAATGTGTTXXXX	\\	&	XX	\\
(10,0) Side 3 Position 1	&	CCGGACTTCCATGTTACTTAGGTCCCAATAGGTTXXXXXX	\\			
(10,0) Side 3 Position 2	&	TAATGCTATTCCATATAACGACCCCCGGTTTTXXXXXX	\\			
(10,0) Side 3 Position 3	&	ACCCAAATCAACGTAAACCGGATGATTGCCGGTCAGTTGTAAATTTT	\\	&	TTXXXXXX	\\
(10,0) Side 3 Position 4	&	TACATCGGGAGAAACTGAGGAAGGTAAACGTTTXXXXXX	\\			
(10,0) Side 3 Position 5	&	AATTATTCATTTCAATGAAATACGCTGGCTTXXXXXX	\\			
(10,0) Side 3 Position 6	&	AAAGTTTGAGTAACATAACGTTATCACTAACAGGGAAGAATTXXXXX	\\	&	X	\\
(10,0) Core Strand 1	&	CCCAAATCAAGTTAAGAATTGAGTCAGGGCGA	\\			
(10,0) Core Strand 2	&	TTACCGAAGCCCTTTTTGGAACAAAATACATATTTTATAAAGGTAAT	\\	&	AGCCC	\\
(10,0) Core Strand 3	&	CTTTACAGCCGATTTAGAGCTTGATTGAGGATTTAGAAGTAAACAGA	\\	&	G	\\
(10,0) Core Strand 4	&	GAGATAGGGTTGATTTTTGTTGTTCCAGTTTAAGAAAAGTTTTTAGC	\\	&	AGATAGC	\\
(10,0) Core Strand 5	&	TGTCACAAGAGAGAGTGCAGGCGCTTTCGCTA	\\			
(10,0) Core Strand 6	&	GTGAGGCGGTCAGTATTTTAACACCGCCTCGTCAATAGTTTTAATAC	\\	&	AT	\\
(10,0) Core Strand 7	&	CTGGCCTTTTTCTGTAGCCAGCTTTCATCAACATGAGATTTG	\\			
(10,0) Core Strand 8	&	TCAGCGTGGTGCTGGTCTTTTGTCAGCACCTGATATTTTTTGTGTCG	\\			
(10,0) Core Strand 9	&	AAAAGGGTCAATAACATTAGAAGGCGGCTTCGCATGCAAATCAACAG	\\	&	TTG	\\
(10,0) Core Strand 10	&	CCGCTACAGAAAGGAAACTAATAGATTAGAGC	\\			
(10,0) Core Strand 11	&	GGGCGCGGTTGCGGTCAGGGTGGCGGTCC	\\			
(10,0) Core Strand 12	&	GCTTACGGATCTTTGATTGTGCCCTTCACCGC	\\			
(10,0) Core Strand 13	&	GATCTTTTCACTGTAGATGGGCGCATCGTTTTTACCGTGCATCCAGA	\\	&	CGG	\\
(10,0) Core Strand 14	&	GCTCATTCAGTGAATAAGGCTTGGCTGACCTTTCCCGGA	\\			
(10,0) Core Strand 15	&	GGCAGCCTCCGGCTGTTCCGGCA	\\			
(10,0) Core Strand 16	&	CATCAATATAATCCTGTCAGATGAATATTTTT	\\			
(10,0) Core Strand 17	&	AACGTGGACTCCAACGTCACCAGT	\\			
(10,0) Core Strand 18	&	AATGGGTACGAACAAAGTTACCAGATCAAAAGGGCAACAT	\\			
(10,0) Core Strand 19	&	AAAGACAAAAGGGCGACATTCAAAACGCAAA	\\			
(10,0) Core Strand 20	&	CCAAGCGCGGTGGTGCTAAGAACTTTGAAAGA	\\			
(10,0) Core Strand 21	&	TAGGCTGCCCTGACTTTTAGAAGGACAGATGAACGGTGTTTTTCAGA	\\			
(10,0) Core Strand 22	&	ATTCGCGTAAATCCGCGACCTGCTGTAGAACGCCAGGCGCA	\\			
(10,0) Core Strand 23	&	TATCCAGAGCACATCAGTAATCTTGACAAG	\\			
(10,0) Core Strand 24	&	CTCGTATTATTTTATCCTTTGCCCGTATCATTTTGCGGTTTTACAAA	\\	&	GA	\\
(10,0) Core Strand 25	&	GCAGCAAATGAAAAATCAGTAACA	\\			
(10,0) Core Strand 26	&	CCGTCTATTAAGCCCAGGATAAGAATACGTGGTGAGTGAGTCACCGA	\\	&	C	\\
(10,0) Core Strand 27	&	CGGGTTACAATCGTTAGCCCCCTGAGCACCATCTGTTCTTGAAATTA	\\	&	TTCATTAA	\\
(10,0) Core Strand 28	&	ATAAAAGACCGATTGAGGGTTTTGGGAAGGTAAATATTGACG	\\			
(10,0) Core Strand 29	&	TTTCCCAGATTTCAACAAATTCATATGGTTTA	\\			
(10,0) Core Strand 30	&	AAACACTCCTGGAGGTTTTAATCATTGTGAATATGGTTTA	\\			
(10,0) Core Strand 31	&	GGAACAAAACAACCCGGATAGGTCGGCTCATTTTCTGGTGACGAGTA	\\	&	GTAAATTG	\\
(10,0) Core Strand 32	&	GCTGAACCAAAGGAATAATGGGTAAAGTTAAAAGAACTCAAATTGCG	\\	&	T	\\
(10,0) Core Strand 33	&	AAGTGTAGGAGCGGGCACCACACCGTACCTTTTAAAGGGAAAATTAT	\\	&	TTGCACGT	\\
(10,0) Core Strand 34	&	AACCACCAGAGGGTTTTTAGAACCTACCATATCA	\\			
(10,0) Core Strand 35	&	GCGCATTAAGCACTGACATTCATTAGTCGTGTTTTGATTATACTTCT	\\	&	GAA	\\
(10,0) Core Strand 36	&	CCACATTAAAAATACTCATATTCCTGATTAATTGTTTG	\\			
(10,0) Core Strand 37	&	TGAAGTCAGATCTAAATGTTTATCGATTATTTATTCACCAACCGAGT	\\	&	A	\\
(10,0) Core Strand 38	&	GGAGCCTCAACGCCTGTAGCATTTTTCCACAGACAGCCCAGCTGCAG	\\	&	CGTGCGGCGTTGC	\\
(10,0) Core Strand 39	&	CGCGTCCGTGAGCCTCTTTTTCACAGTTGAGGATCC	\\			
(10,0) Core Strand 40	&	TTAATGAATTTTTGGCCAACGCGCGGCGGGCCGGGTACCGAGCTC	\\			
(10,0) Core Strand 41	&	GAACCCATGTACCGTTAGCAAGCAGCCACCACCGGAAACCCGCCACG	\\	&	TCATAGCT	\\
(10,0) Core Strand 42	&	ATCAACACGGAAAAAGAGTTTTGCAGAAAGTATCGGCCCATTCAG	\\			
(10,0) Core Strand 43	&	TGTTAAATCAGCTCAAAATCCCAACGCGGGCTGCGC	\\			
(10,0) Core Strand 44	&	AACCAATCCCTGTTTGCTCATTAGTTGGGGATCGGT	\\			
(10,0) Core Strand 45	&	ATTAGTAATAACATGCCTTGCTGGTAGAT	\\			
(10,0) Core Strand 46	&	TTTTAGACAGGAACTTTTGTACGCCAGAATCCTGAGAA	\\			
(10,0) Core Strand 47	&	TATCAGAGAGTCAGAGAGCACCGTAATCAAATGTTTTGTCCAGGGCA	\\	&	G	\\
(10,0) Core Strand 48	&	AAGCATAAAGTGTAACATTAATTCTCACTGC	\\			
(10,0) Core Strand 49	&	GGGATCAGCCAGCGGTAATTTTCTGCCAGCAC	\\			
(10,0) Core Strand 50	&	GAAAATCCTGTTATTTGCAGCAAGTTTTTCTTTGCGTAT	\\			
(10,0) Core Strand 51	&	AATCGGCGGAATTTGGTTTCCTGTGTGAAATAATCATGGGGAACGGA	\\			
(10,0) Core Strand 52	&	CAGCGGAAGCTGGCGAAAGGGGTTTTTGTGCTGCAAGGCGATTAAGT	\\	&	TTGTAAAAAGTGCCAA	\\
(10,0) Core Strand 53	&	GCACCGTCGAAACAAAGACCAACTACGTTGGTCCAGCCAGCTTTCCG	\\	&	G	\\
(10,0) Core Strand 54	&	ACACCAGACCGGAAACCAGGTTTTAAAGCGCCATTCGCTCAGGAA	\\			
(10,0) Core Strand 55	&	GGGGTAATAATAGTTGATTCCCATAGCTGAATCAATACATAAAA	\\			
(10,0) Core Strand 56	&	TGCCGAGCTGAGTAGAGCGGGCCTCTTCGCTGGAAGGGCCGGTTGTG	\\			
(10,0) Core Strand 57	&	TAATATTTAGCAAATACCAAGTTACAAAAGACAATAATCGGCCCCAG	\\	&	C	\\
(10,0) Core Strand 58	&	TTTAGCGTGAACAAGAAAAATTTTATATCCCATCCTAAACGCTCAGC	\\	&	CATATCC	\\
(10,0) Core Strand 59	&	CGCTGCGCGAACGGGTAACAGGAGTGGAAATATTTTTACATTCGTGC	\\	&	TTTCCTCGTTA	\\
(10,0) Core Strand 60	&	GTGCCGTAAGACGGGAACCAACGCTAACGAGTTTATCCTAAAAGG	\\			
(10,0) Core Strand 61	&	CTAAAACATCGCTCAGAATGGCTTGGCCAACACCAGTAA	\\			
(10,0) Core Strand 62	&	ACATTTCGGTGCCTAAAAAGAGTCTGTCCATCGTGAGGCCGTCACAC	\\	&	G	\\
(10,0) Core Strand 63	&	TATAATCAACGCAAATTCAATCGTCTGAAATGAACAATAGTAATGCA	\\	&	G	\\
(10,0) Core Strand 64	&	TGAATCTTATAAGTCCAACCTCCCGACTTGCGGGAGGTTTAATCAAG	\\	&	AAACGCGCC	\\
(10,0) Core Strand 65	&	ATCTCCAAAAAAAAGTAAAGGAGTAAATG	\\			
(10,0) Core Strand 66	&	GGGTTTCTGTATGGGATTTTTTTTCTAAACAACTTTCAACAGCC	\\			
(10,0) Core Strand 67	&	ATGTTTACCAGTCCCGAAACGTATAACCTCACCCTCATTGAACCGCC	\\			
(10,0) Core Strand 68	&	CCTCAGAGCCGCCACCCTCAGAACTATCGAGGTGAATTTCACCCTCA	\\	&	G	\\
(10,0) Core Strand 69	&	GATAAAAATTTTTAGAATACTTGCAAAGA	\\			
(10,0) Core Strand 70	&	ACTCCAACAGCCCGAAGTTGAGATATTGACCGATTAGCAAAATTAAG	\\	&	CAATATTTTAGCCTC	\\
(10,0) Core Strand 71	&	CCTAAATTAGAAAAAGTGAGAGACGCAAAAGAAATGGAAAAATCATT	\\	&	ACCGCGCCATTCCAA	\\
(10,0) Core Strand 72	&	AAAATATCTTTAGGAGTAATTTTACGCCGCGCGGGAGCTAATTAAAC	\\	&	CAAGTTTTTCCGCACTCATCG	\\
(10,0) Core Strand 73	&	TATCCGGTATTCTAAGAACGTTTTAGGCGTTACAAGCAAGAACAAT	\\			
(10,0) Core Strand 74	&	GTAACAGTTTCGGTCATAGTCCCTAATTTCCCTTTCCTTA	\\			
(10,0) Core Strand 75	&	GGAAACCTGTCGTGCCTCATAGTTAGACGTTAATTGCGAA	\\			
(10,0) Core Strand 76	&	TCATAATCGGAACAACGCTCTTTTAAAATGCGTTTCAGCGGAGTGTT	\\	&	TTGAATAGAAA	\\
(10,0) Core Strand 77	&	ATATAAGTGGGGTTTTCACCCTCAGAGCCGCCACCGGACGATAGT	\\			
(10,0) Core Strand 78	&	TCACGACGTGGGTAACGTGAAGGGATAGCTCTTTCTACTACAGGCAA	\\	&	GTTGCGGGA	\\
(10,0) Core Strand 79	&	GTAAGAGCGACCCTGTAACCCTTTTTTATAATCGCTAAATCGGT	\\			
(10,0) Core Strand 80	&	CATTGCAACAGGAAAATTTACGAGTCCTTATCCAATAGCA	\\			
(10,0) Core Strand 81	&	AGTAATAAATTTAACAATAGCGATAGCTTAGACCTTGCACCCAGC	\\			
(10,0) Core Strand 82	&	TGAATAATTAAGACCTGTACCGACAAAAGGTAAAGTATATTTTGC	\\			
(10,0) Core Strand 83	&	ACGGGGTCAGTGCGCAGACGTAGCGACAGAATTAATAATTCCTTATT	\\	&	A	\\
(10,0) Core Strand 84	&	GAGGAAGTTTCCATTCATCGCCCGTACTCAGCTTGATACACCGCCTC	\\			
(10,0) Core Strand 85	&	CGTTTTAATTCGAAGTACCACATTATTACAGGGAAGCCTTGCCAAAA	\\	&	G	\\
(10,0) Core Strand 86	&	TCAGGCGGAATATTCAAACATTATAACACTATCATATTTTCCCTCGT	\\	&	TTACCAGACG	\\
(10,0) Core Strand 87	&	GAAGTTTCGTAGCTCAGAAGTTTTGCCAGAGACGATAA	\\			
(10,0) Core Strand 88	&	GATAATCAGAAAAGCAACCGTTCATTCTGCGGCCGGAGAAAACCAAA	\\			
(10,0) Core Strand 89	&	CAGAGGCGAGCAAATCATTTCATTTGAATTACCTTTTTT	\\			
(10,0) Core Strand 90	&	ATCGTAGGCAGTACATAATTTTTCAATATATGTGAG	\\			
(10,0) Core Strand 91	&	CAGTCAATTTTAAAGGGGCGCGAGCTGTTTTAAGGTGGC	\\			
(10,0) Core Strand 92	&	CTGAACAAAGATAACCTGACCTGAAAGCGAACCCGCTTTCGTCTTTC	\\	&	CAGCGTAACCGTTGAAA	\\
(10,0) Core Strand 93	&	GAGGCGGTCAGCGCCCACCAGTTTCAGGGAAACACTGAATCGGTTT	\\			
(10,0) Core Strand 94	&	GAACACTCCATCCAATAAATCATAATAGTAGTAACGCAAG	\\			
(10,0) Core Strand 95	&	TACATCGATGATATTCTTTCATTTTGCAATGCCTGAGTAATGTGTAG	\\			
(10,0) Core Strand 96	&	ATAGCGAGAGGTTACATTTAACAAGAGATTCGTAAATAT	\\			
(10,0) Core Strand 97	&	CTTTAGTGATGAAAACATATTACCGCTGTCTTCATGTAGAAGAAGGC	\\	&	T	\\
(10,0) Core Strand 98	&	TTGCCCTGTTTGAGGAGCTGAGGCTTGCAGGGATTTTTTAAAGGCCG	\\	&	CAGTGTCTCCCTTAC	\\
(10,0) Core Strand 99	&	GAATTTACCAACGGCTACAGAGGCCGGCTGGT	\\			
(10,0) Core Strand 100	&	GGTCTTTACCCTGACTTAATCGTAAAACTAGCCAAAAATA	\\			
(10,0) Core Strand 101	&	TTAACTTGATTTAGAAAGTACCAGGAAGATTGTATATGTTAAAA	\\			
(10,0) Core Strand 102	&	TTGAGCCATTTGGGAATATCACCGCTAACTCAAGCCTGGG	\\			
(10,0) Core Strand 103	&	TGGGCGCGCGGGGAGCTCACAATTCCACACAATTTTATACGAGCCGG	\\			
(10,0) Core Strand 104	&	GTCTGATGGTGGTTCGGAATAAGTTTATTTCCAGCGCCGAATTCGTT	\\	&	GTTATCC	\\
(10,0) Core Strand 105	&	TCAAATATAGATTTTCAGGTTTAAAATAAAGAAACTATCGCACTTGC	\\	&	C	\\
(10,0) Core Strand 106	&	TTGACGCTAACCGTTGTAGCTTTTTACTTCTTTG	\\			
(10,0) Core Strand 107	&	ACAAAGCTAACTGTTGATTACGCCTCAAACTTAAATTTCT	\\			
(10,0) Core Strand 108	&	ATCAGCTTGCTTTTTCAGCATTAACCAATAGTAGACTT	\\			
(10,0) Core Strand 109	&	GACAATGACAACAACACAAACTATTAATTGTGTTTCGT	\\			
(10,0) Core Strand 110	&	GCTTTCAGAGGTGGAGTCTCCGTGGCCAGGGTTGAGAGA	\\			
(10,0) Core Strand 111	&	TTCTGTAAATCGTCGCTATTAATTTAGAATCCCAGACGACGAGGCAT	\\	&	TTGAACACC	\\
(10,0) Core Strand 112	&	AAAGCGAATGCAGATACATAACCGCCACCCTCGTACCGCCGCCGTCG	\\	&	AAAAATACG	\\
(10,0) Core Strand 113	&	TGCGTTATATTTTAGTTAATTTCAAAACGATTTTTTGTTTAACGTCA	\\	&	TTTTAATGAAA	\\
(10,0) Core Strand 114	&	AATTGCTCCAAAGCGGATTGCATCGTCTGGAGCAAACAAGAGAATCG	\\	&	TTTTGAACGG	\\
(10,0) Core Strand 115	&	GCCAACGCACAAAGAACGCGAGAAATAGCAGC	\\			
(10,0) Core Strand 116	&	AAGGTTTCTTTTTTGCTCGTGGAACGTTTTGGGTAGCGTTTTTCCAG	\\	&	TAAGCGTCATACATG	\\
(10,0) Core Strand 117	&	CCTATTATTCTGAAACATTTTGAAAGTATTAAGAGGCTCAGTCTCT	\\			
(10,0) Core Strand 118	&	TTAGTTGCATTCTGTCTTGAAAACACGCCAACATGTAATTTAGCTTG	\\	&	A	\\
(10,0) Core Strand 119	&	TAATGCCCGAGTGTACCGTCAGACCAGGTCAGACGATTGGTGACAGG	\\	&	ATTTCGGAA	\\
(10,0) Core Strand 120	&	TTAAACAGGAGGTTTAAGAGCCACGCTCAGTACCAGGCGGATAGCTT	\\	&	C	\\
(10,0) Core Strand 121	&	TGTATTTTCAAATTGAATCCCTGCGGAAATTAGAGAGTACCTTT	\\			
(10,0) Core Strand 122	&	AACTTTTTTTTAAATATACAATTTTTCTTACCAGTATAAA	\\			
(10,0) Core Strand 123	&	ATTATTTTTTCAGAAGCTTTTGATTTTAGAGGTCATTTTTGCGGAT	\\			
(10,0) Core Strand 124	&	AGCTATATGCAAATGGTGAGAAAGAACGAGTATTGCAAAAACATGTT	\\	&	TTAAATAT	\\
(10,0) Core Strand 125	&	TTATTTTTTTCTAACCTCCCATAGGTCCCTGTTTAGTATCATA	\\			
(10,0) Core Strand 126	&	TGATACAGCCTGCCTAGGTTGAGGTGTAGCGC	\\			
(10,0) Core Strand 127	&	TAAGAGGAAGGTCAGGTCGTCATATTAGGAAT	\\			
(10,0) Core Strand 128	&	AAAAATCAGGCTTAGAGTTTAGACTGGATATTTTCGTCCAATA	\\			
(10,0) Core Strand 129	&	AACGCCATATGTCAATAGGGTAGCCAGTTCAGAAAACGAG	\\			
(10,0) Core Strand 130	&	GCACGTTAAATAAGAACATCAAGAAAACAAAA	\\			
(10,0) Core Strand 131	&	ATCGCAAGTCAACAGTGAGTCAATAGTGAATTTTTTTTCAAAAT	\\			
(10,0) Core Strand 132	&	GGAAAGCGGAGACTCCAGAGCCGCCGCCTTTTGCATCCTTGATTTTA	\\	&	TTCACAAACAAATAAATCCTC	\\
(10,0) Core Strand 133	&	GTGATAAATAAGGACTTTTTCGCG	\\			
(10,0) Core Strand 134	&	TAATTACTTAATGGTTTTACCTGATACCTTTT	\\			
(10,0) Core Strand 135	&	GGCTTAGGTTTTTGGGTTATATAACTATA	\\			
(10,0) Core Strand 136	&	TTGAAACGCAATAATAACTCTGTGACGGTCTTTTTACCGGGATCCAG	\\	&	CGCTTTTGC	\\
(10,0) Core Strand 137	&	AAAATCATTTTCGGAACCAGAGCCACCACCAGAAATTAGGTGTATCA	\\	&	CCACGCATA	\\
(10,0) Core Strand 138	&	TAATGCCACTACGAAGAACTAACG	\\			
(10,0) Core Strand 139	&	CCCTCAAATTTTTCTTTAAATATTTTTGTTTTGAGATCTACAAAGGC	\\	&	TA	\\
(10,0) Core Strand 140	&	GAATTTTTAGAGCTTAATGCGATATTATTTATCCTCA	\\			
(10,0) Core Strand 141	&	GGGAGCCCAGAGAATAAATTTGCCAGTTACAAATTTTTAAACAGCC	\\			
(10,0) Core Strand 142	&	AACAATGAAATAGCAACCTTATTACATCAGAC	\\			
(10,0) Core Strand 143	&	AGCGAAAGACAGCATCCATAAACAACTTTTTCGCGCCTGTGC	\\			
(10,0) Core Strand 144	&	AAAGAGGCAAAAGAATGGCAACAGCTGATGGA	\\			
(10,0) Core Strand 145	&	CGGGGAATTTTCCGGCGAACGTGGCGAGGGTTTTGCGTACTAT	\\			
(10,0) Core Strand 146	&	AGAAGATAATTAGACTTTCGACAAGGTTGCTTTGACGAGC	\\			
(10,0) Core Strand 147	&	CGTCTTTCCAGAGCCTACATAAAACAAATCCA	\\			
(10,0) Core Strand 148	&	TTTAATGCAATTATCACGAACGAACCACCAGC	\\			
(10,0) Core Strand 149	&	AGCCGTTTTGTAAATGGCTGAGAAAGGGCTTAATTGAGAA	\\			
(10,0) Core Strand 150	&	TAATGGAAAGGAGCGGGCGAACAATTACAAACTGATAGCC	\\			
(10,0) Core Strand 151	&	AAACAACATGTTCAGCGAATTAACTTCGAGCC	\\			
(10,0) Core Strand 152	&	CACAGACATGGCAATTTGGCCCACTACGTGAA	\\			
(10,0) Core Strand 153	&	GCCACCATCGATAGCGGTAATTGAAGTTTTA	\\			
(10,0) Core Strand 154	&	AGGTGAATTTAGAGCCAGCAAAATCAAAGGGCGAAAAA	\\			
(10,0) Core Strand 155	&	CAAGTTTGTCGGCATTGCCCGTATAAACAGT	\\			
(10,0) Core Strand 156	&	GTCACCAATGAAGGTACGGCATAGCAAGA	\\			
(10,0) Core Strand 157	&	GTTCAGCACTGCGTCACCCTCAGCGCTTTTGA	\\			
(10,0) Core Strand 158	&	ACGGAATACCCAATTTTAGAACTGGCATGAACGTAGAAGAGTCCACT	\\	&	ATTAAAG	\\
(10,0) Core Strand 159	&	ACCGATATATTCGGTCCTAAAGACGCCAGAAT	\\			
(10,0) Core Strand 160	&	ACGCTGGTGACACCACCGAAATCGGCAAAATC	\\			
(10,0) Core Strand 161	&	CCACCACCTCAAGAGAAGGATTAG	\\			
(10,0) Core Strand 162	&	CCGTTTTCGTGCTGCGGCCAGAATATGAGCCGCAGCAGGC	\\			
(10,0) Core Strand 163	&	AGAACCGCCACCCTCAAAACGGGTGAGGGTTG	\\			
(10,0) Core Strand 164	&	CTGGCCCTTCAATAGAGTCCAGCATCAGCGGG	\\			
(10,0) Core Strand 165	&	TAAGTTAATAAAACGGCACCAACAAATATCG	\\			
(10,0) Core Strand 166	&	GGCTTGAGTACCTTATGCGATTTCATCCCACGCAACCA	\\			
(10,0) Core Strand 167	&	TAGAAAGATCAACTAACCAGACCGGAAGCAA	\\			
(10,0) Core Strand 168	&	AGAAAAATCTACTGGTCGGATTGATTATA	\\			
(10,0) Core Strand 169	&	AGCGAGTACGGTCATTGCCTGAGAAAAAAGAT	\\			
(10,0) Core Strand 170	&	TATCATCGGCAACCGCAAGAATGCCAACGGCA	\\			
(10,0) Core Strand 171	&	AGAGCATAAAACCTAAATTAATGCCGGAGCATATGTACATAAATC	\\			
(10,0) Core Strand 172	&	TCCGTTTTTCATCAAGCTCATAACGGAACGTG	\\			
(10,0) Core Strand 173	&	AGTAAAATGCTTAATTGCTGAATA	\\			
(10,0) Core Strand 174	&	ACGAGGCGTGCCAGTTTGAGGGGACGACGACATTTTTTAATCGTCGC	\\	&	T	\\
(10,0) Core Strand 175	&	GTAAAAAAAGCCGCACTACATTTCCCCAAAAAGGTGTCTG	\\			
(10,0) Core Strand 176	&	CGATGCTATTCATTCAAACCCTCAATCAA	\\			
(10,0) Core Strand 177	&	GTATTGCTTTGAATATTTAAATTCCGACCGT	\\			
(10,0) Core Strand 178	&	AAAACAGACGTCAGATGAATATACTAAAGCATCACCTT	\\			
(10,0) Core Strand 179	&	AGATGATGAAACAAATAAACACCGGAATCA	\\			
(10,0) Core Strand 180	&	AGAACAGGATTCGCCTGAACCGCTAGGGGTTATCT	\\			
(10,0) Core Strand 181	&	AGCGAAAGCGGCAATCCAAATAAGTCTTCTGA	\\			
(10,0) Core Strand 182	&	GCAACAGTGCCACGCTGAGAGCCA	\\			


==> MonomerSequence-6_0.tex <==
Name & Sequence \\
\hline
\endfirsthead

Name & Sequence \\
\hline
\endhead

\endfoot
\endlastfoot
(6,0) Side 1 Position 1	&	CGTATAACTAAATCGGAACCCTAATTXXXXXX	\\			
(6,0) Side 1 Position 2	&	TAACAACAAAGTACCGACAGCAGCGCATTATTXXXXXX	\\			
(6,0) Side 1 Position 3	&	GAACCCTTCTGACCTAATTTTTTGGGGTCGATTXXXXXX	\\			
(6,0) Side 1 Position 4	&	AAACGTCACCAATGAAAGAGCAAATATCAGATTXXXXXX	\\			
(6,0) Side 1 Position 5	&	ATAATCAAAATCACCCGGTCATAGTAGCGCGTTTTGATGTCGTTAAC	\\	&	TTXXXXXX	\\
(6,0) Side 1 Position 6	&	TTAGCAAACGTAGAATTATTACATCTTACCAAACATCCTTXXXXXX	\\			
(6,0) Side 2 Position 1	&	AATCCCTTCCGAGGAAACGCATTTGTATGAGCTTXXXXXX	\\			
(6,0) Side 2 Position 2	&	TTAAGAGGGGCGGATAAGTGCTAGAAAGACTTXXXXXX	\\			
(6,0) Side 2 Position 3	&	TTCTTTTCACCAGTGAGGTGCGCTTTCGCACTTXXXXXX	\\			
(6,0) Side 2 Position 4	&	AGGCAGTTTCCAAGTAATCATTGTGAATTCGAAGGCATCATGAGGTT	\\	&	XXXXXX	\\
(6,0) Side 2 Position 5	&	TTAGGAATACCACATAACATTATGTTAATAATCAGAAGATTAAATTT	\\	&	XXXXXX	\\
(6,0) Side 2 Position 6	&	TGTGTCTTTTAAATCCGCGACCTGCTCCAAGAATACTCTGGCCTTTX	\\	&	XXXXX	\\
(6,0) Side 3 Position 1	&	TAACGGAAACAACGGAGATTTGTCCGCATTAATTXXXXXX	\\			
(6,0) Side 3 Position 2	&	TGATAAGCTCAACATGTTTCATACGGTAATTTXXXXXX	\\			
(6,0) Side 3 Position 3	&	TGGCTGACCTTCATCACCAGGCTTAAACGAAATCAACAAATTGTATT	\\	&	XXXXXX	\\
(6,0) Side 3 Position 4	&	AACGGATTCGCCTGATATCTAAAAAAAACAGTTXXXXXX	\\			
(6,0) Side 3 Position 5	&	CCTGAGCAAAAGAAGCGTGTGAGCTGGCATTXXXXXX	\\			
(6,0) Side 3 Position 6	&	ATTATCATTTTGCGGAAAAGTTTAATAGATGGAAGAAATTXXXXXX	\\			
(6,0) Core Strand 1	&	CCAGAGCCTAATTTGACAGGGAAAGACAAAG	\\			
(6,0) Core Strand 2	&	GCGCGAACTGATTATCAACCACCAGCAGAAGA	\\			
(6,0) Core Strand 3	&	TTTTTATTAAATCCAGTGAATTTGAGAATCGCCATATT	\\			
(6,0) Core Strand 4	&	ACCTACCAATATTCCTGACTCGGACAATAGCCCTAAAA	\\			
(6,0) Core Strand 5	&	TGTTCAGCTAATGCATGAACACCAGTAATAA	\\			
(6,0) Core Strand 6	&	CAATATTTAATCCTGAATGGCCCACTACGTGA	\\			
(6,0) Core Strand 7	&	TGCCGTAATCAGTAGGAGCGCTAATACAGGA	\\			
(6,0) Core Strand 8	&	ACCGACTTCCAGTAGCACCATTAGTCAAAGGGCGAAAAA	\\			
(6,0) Core Strand 9	&	TCAGACTGCCCCCTGTCAGTGCCTTGAGTA	\\			
(6,0) Core Strand 10	&	CGATAGCAGCACAGCTCAGCAAAGAAACAAT	\\			
(6,0) Core Strand 11	&	CTTACACTGATATATATTCGGTCGTTCCAGTA	\\			
(6,0) Core Strand 12	&	AAGACTCCAATACATAGAGTCCACTATTAAAG	\\			
(6,0) Core Strand 13	&	TACCGATAGTTGCGCCTCAGCAGCAATCCTCA	\\			
(6,0) Core Strand 14	&	GTCCACGCAAGTTTATTTCCGAAATCGGCAA	\\			
(6,0) Core Strand 15	&	AGAGCCGCTGAAACATGAAAGTA	\\			
(6,0) Core Strand 16	&	GCCAGAATCCTGTGCACTCTGTGGGGTTGCGGCCCCAG	\\			
(6,0) Core Strand 17	&	CACCGTACTCAGGAGGTAGCAACGGTTTTGCT	\\			
(6,0) Core Strand 18	&	CCGCCTGGCATATGGTTGGAGGTGTCCAGCA	\\			
(6,0) Core Strand 19	&	GATAACTGGCTCATTAGACTTTTCAAAGCGG	\\			
(6,0) Core Strand 20	&	ATAAGGCTAATTGGGCTTGAGATGTGGTGCCATCCCAC	\\			
(6,0) Core Strand 21	&	AATCTACTACAGGTCCCGAAAGACTTCAA	\\			
(6,0) Core Strand 22	&	TGCGATTTTAAGTCTCATCAACCCAACCT	\\			
(6,0) Core Strand 23	&	TCCTGTAGGTAGGGTAGCTATTTTAGGTCTTT	\\			
(6,0) Core Strand 24	&	CACTCATCTCAGCAGCAACCGCAAGAATGCC	\\			
(6,0) Core Strand 25	&	ACAGGCAAGGAAGCAAATCACCATCAATATCGATGATGAATCCC	\\			
(6,0) Core Strand 26	&	CGGCAAACAGAGGACACCAGAGCACATCCTCA	\\			
(6,0) Core Strand 27	&	ATAGCGACTTTAATTGCTCCTTT	\\			
(6,0) Core Strand 28	&	CATCGCCTGGTGTAGATGGGCGCATCGTAACTTAAAATTCGTTTTTT	\\			
(6,0) Core Strand 29	&	ATAAAAAAATCCCGTTTGATTCTCAATCATGAATATAA	\\			
(6,0) Core Strand 30	&	GGGTAAAGGCATAGGCATCAATATCTGGTCA	\\			
(6,0) Core Strand 31	&	TAATACAAAATCGCGAAAGCCCCTAAATAAG	\\			
(6,0) Core Strand 32	&	TTGCGTAGTAACAGTACCTTTTAACCTTGCTGAACCTC	\\			
(6,0) Core Strand 33	&	CAAGAAAACAAAATTTCATAATTACTAGAA	\\			
(6,0) Core Strand 34	&	CAATATTGAATACCAAGTCCACTAGGGCATATCTT	\\			
(6,0) Core Strand 35	&	GCGAAAGGGGTAATAAGAAACGATAATTTAAT	\\			
(6,0) Core Strand 36	&	ACGCTGAGAGCCAGCAGCAAATG	\\			
(6,0) Core Strand 37	&	ACCCAAATCAAGTTGAGTTAAGCCAGGGCG	\\			
(6,0) Core Strand 38	&	GAAGCCCTTTTTAAGGGAACAACATAAAGGTGGCTTTTAACATATAA	\\	&	AAAAAGAATAGCCC	\\
(6,0) Core Strand 39	&	GAGAATACCCGATTTAGAGCTTGTATTAGACTTTACAAGGTGAG	\\			
(6,0) Core Strand 40	&	GAGATAGGGTTTTTTGAGTGTTGTTCCAGTTTAAAAGTAAGCAGATT	\\	&	TTTAGCCGAACAAA	\\
(6,0) Core Strand 41	&	AGAAAATTCCCTGAGAGGGTCATTGCAGAAA	\\			
(6,0) Core Strand 42	&	GCGGTCAGTATTAACATTTTCTGCAACAGTGCCATAATACATTTTTT	\\	&	TATTTAGAA	\\
(6,0) Core Strand 43	&	TTTAACCATTTTGAACGCCATCAAAAATAATTCGCGACTAAAA	\\			
(6,0) Core Strand 44	&	GACTTGTAGAACGTCAGCGTTTTTCTGGTCTGGTTTGACCCCTTTTG	\\	&	ATTATACCA	\\
(6,0) Core Strand 45	&	TTTTAAAGCGAACGTATAACAGAAAAAAAGAATATTTAGTTGAAAGG	\\	&	AATTG	\\
(6,0) Core Strand 46	&	CCGCTACAAAGGAAGTAGAGCCGTCAATAG	\\			
(6,0) Core Strand 47	&	TGCAGGGTTCTTTGTCCATTTTGCGCAGTGTCATACCCAAAAGAACT	\\	&	GTTTTGCATGATT	\\
(6,0) Core Strand 48	&	TCAATCCGCCGGGCGCGCGCCAGGAGCAAGCG	\\			
(6,0) Core Strand 49	&	GCAACCAGTGCCACTAACCTGATTGCCCTTCA	\\			
(6,0) Core Strand 50	&	TGAGGTTTTGACGACGGATTGACCGTAATGGGTTTTTAGGTCACGTT	\\	&	GATAAAT	\\
(6,0) Core Strand 51	&	TCTTGACAAGAACCGGATATTCACTTTGAAGCGGTAT	\\			
(6,0) Core Strand 52	&	CGTCTCGTCGCTGGCATGCTGAT	\\			
(6,0) Core Strand 53	&	TTGTTTGGATTATACTCAATATTTGAATG	\\			
(6,0) Core Strand 54	&	AACGTGGACTCCAACCCATTAGC	\\			
(6,0) Core Strand 55	&	TGCGGCTGTTACCAGAAGGAAAATAAATCAGAAACGCA	\\			
(6,0) Core Strand 56	&	GCGACATTCAACCGATTGAGGGACACGGAAT	\\			
(6,0) Core Strand 57	&	AAAACGAACACCGTCGGGTTTAATTAGCCGGA	\\			
(6,0) Core Strand 58	&	TGACCAATTACCCAAATTTTCAACGACGAGGCGCAGACGGTCATTTT	\\	&	CATAAGG	\\
(6,0) Core Strand 59	&	GCTCATTTAGCGCGAAACAAAGTCGTGCCGGAACCGAAC	\\			
(6,0) Core Strand 60	&	GTTGGCAGCCTCCGGGATGAACGGTGTACAG	\\			
(6,0) Core Strand 61	&	CCTTTGCCCGTTTTACGTTATTAATTTTAACAAAGAAACCACCATTT	\\	&	TAGGAGCGG	\\
(6,0) Core Strand 62	&	AAAAATCTAAAGCATCCATCGGGA	\\			
(6,0) Core Strand 63	&	CCGTCTATCCAATAATAACTACGTGGCACAGATGCCTAATTGGGAAT	\\	&	T	\\
(6,0) Core Strand 64	&	GGCATCAGGTGTGTCAGCGGTGAAGGCCGGCTGCCAGCTGAATTATC	\\	&	ACCGTC	\\
(6,0) Core Strand 65	&	AAGACACGGGAAGGTAAATATTTTTTGACGGAAATTATTCATTAAAG	\\	&	G	\\
(6,0) Core Strand 66	&	ATTAAGTTCGAGAAACTTACCAGCGCCAAAG	\\			
(6,0) Core Strand 67	&	ATACGTAACTTACGGCACCAGAACGAGTAGTATGCCCTGA	\\			
(6,0) Core Strand 68	&	GTGAGCGACCAGCTTTCCGTGGGATTCAACTTATCGCACTCTGCTCA	\\	&	TTCAGTGA	\\
(6,0) Core Strand 69	&	AAATATCAAGGAAGGTTTGCTTTAGTGATGAACTCAAACTGTTTAAC	\\	&	G	\\
(6,0) Core Strand 70	&	AGTGTAGCAGCGGGCGCCACACCCGAAACAATAAAGGGATACAGAAA	\\	&	TAAAGAAA	\\
(6,0) Core Strand 71	&	AATTATCATCTATCTTTTAAATTATTTGCACGTAAA	\\			
(6,0) Core Strand 72	&	GACGGGAAAAGCACCTGGCCAATCTTTAATGTTTTTATAATGGAAGG	\\	&	GTTAGA	\\
(6,0) Core Strand 73	&	ACCAAATACCGAACGAGATGATGGCAATTCATTCTGAAT	\\			
(6,0) Core Strand 74	&	CCTTAGAATTCCACAGTCAACAATTTACATTGCAGTCACGAGTAAA	\\			
(6,0) Core Strand 75	&	AACACTGAGTTTCGTTTTTCACCAGTACAAACTGTCGTGCCGGGATT	\\	&	GATTATTT	\\
(6,0) Core Strand 76	&	ACGCGTGCCTGTTCTTCGCTTTTGTCCGTGAGCCTCCTCAC	\\			
(6,0) Core Strand 77	&	AGCTGCATTAATTTTTGAATCGGCCTGCTGCGAGTTGAGGATCCCCG	\\			
(6,0) Core Strand 78	&	CCACCCTCATTTTCAGGGCCACCCTCTCAGAACCCGCCACGGTGCCA	\\	&	ATCGTAAT	\\
(6,0) Core Strand 79	&	TGTTTAGTGGTGAAGGGATAGTTTTCACGGAACGTGCATCGCCGGAA	\\	&	A	\\
(6,0) Core Strand 80	&	AACGTTAATATTTTGACATCGACTGCCGTTCCCAGGCA	\\			
(6,0) Core Strand 81	&	CAATAATCAGTAGATTCAAACTTACATTTGCTCAGGCT	\\			
(6,0) Core Strand 82	&	GTAATAACATCACTTGCTGGTAATATATT	\\			
(6,0) Core Strand 83	&	TTTAGACAGGAACGGTTTTTCGCCAGAATCCTGAGAAGT	\\			
(6,0) Core Strand 84	&	GAGATAACGGGTAATTCGACAGAATCAAGACAACAGCCCTCGCTTCA	\\	&	C	\\
(6,0) Core Strand 85	&	GAGCCGGAAGCATAATAACTCACCGTTGCGC	\\			
(6,0) Core Strand 86	&	AACCGGCCGGGTTACCGTTTTGTCCATACCGG	\\			
(6,0) Core Strand 87	&	CAGGCGAAAATCCGCGGAGTTGCGTGGTTTGCGGTTTG	\\			
(6,0) Core Strand 88	&	GGAACGGAGCGCCATGCATGGTCATAGCTGTTGCTCGAATGCTTTCA	\\	&	G	\\
(6,0) Core Strand 89	&	CGGTGCGGGCCTCTTCGTTTTTTACGCCAGCTGGCGAAAGGGGCCAG	\\	&	GGTTCACGACGT	\\
(6,0) Core Strand 90	&	AACGGCAGAGAGGCAAATGTTACTACAAACGGCGACAGTATCGGCCT	\\	&	C	\\
(6,0) Core Strand 91	&	TAACAAAGCCAGCCAGCTTTCTTTTGGCACCGCTTCTGGTTGCCAGT	\\	&	T	\\
(6,0) Core Strand 92	&	AATTTATTTAGAAGAAGCGCAACTGTTGGGAATTCGCCATCGCCAGC	\\	&	A	\\
(6,0) Core Strand 93	&	GAAGATTGTAATCAGACAGAGGCGAATTACCAGGCTGTCTGCCCTGC	\\	&	T	\\
(6,0) Core Strand 94	&	CGAACCTCAAGAAAAATAATATTTTTTCCTAATTTACGAGCTCATGG	\\	&	ACCGCCAGAA	\\
(6,0) Core Strand 95	&	GCTGCGCGTATTAAACACAGGAGGAATACCTATTTTTTGACGGTGCT	\\	&	TTCCTCGTTA	\\
(6,0) Core Strand 96	&	GGTGCCGTGAATTAACGCTAACGAGCGTCTTTCCTGAATCGGGACAT	\\	&	T	\\
(6,0) Core Strand 97	&	CATCGCCATTAAATCGCTATTAGCAGAGATATAATAAAA	\\			
(6,0) Core Strand 98	&	GCAGATTTGCCTGGGGAGAGTCTGTCCATCAAGGCCACCACGACCAG	\\			
(6,0) Core Strand 99	&	AATCAGTGCGCAAATTTCTGAAATGGATTATAGATAAGGAACGCGC	\\			
(6,0) Core Strand 100	&	TTACCAACTCCTGAACCCGACTTGCGGGAGGTTTTGAAGAGATTAGC	\\	&	TGTTTA	\\
(6,0) Core Strand 101	&	AACAACTAAAGGAATAACTTTCATCTAAA	\\			
(6,0) Core Strand 102	&	TTCACGGTGTCTTTCCAGATTTTCGTTAGTAAATGAACTT	\\			
(6,0) Core Strand 103	&	AATCGGCGAAACGTACATAACCTCAAGGTGGAGCGCCACCCTTTAGT	\\	&	AC	\\
(6,0) Core Strand 104	&	CGCCACCCTCAGAACCGCCATCACAAAGGCTCCAAAAGCGCCACC	\\			
(6,0) Core Strand 105	&	CCCTGTAATACTTTTGCATAAAACTAATA	\\			
(6,0) Core Strand 106	&	ATATCGCGTATTATAGAACGAACTACCCGTCGGTAGTAGCATTAACA	\\	&	TCCAATTTTTAATCAT	\\
(6,0) Core Strand 107	&	GGTTTGAATTTAGTATTTAACCTCACAAACATTCAATATAATTACCG	\\	&	CGCCCAATGAACGGG	\\
(6,0) Core Strand 108	&	GGAGCTAACAAGTACCGCACTTTTCATCGAGAACAA	\\			
(6,0) Core Strand 109	&	CGGTATTCTAAGAACGCGATTTTTTTTAGTTTGCCGGCAATAT	\\			
(6,0) Core Strand 110	&	TTAACGGGTATTAGCGTTTAAACACTTGAGCCTGAAATCA	\\			
(6,0) Core Strand 111	&	CCAGTCGGGAAACCTACAACGCGCGTAACGAACAGTTT	\\			
(6,0) Core Strand 112	&	GGGTAACGGATGTGCTAGATAGACTTTCTCCGCTATATTCAATTCTG	\\	&	CTAAATC	\\
(6,0) Core Strand 113	&	TCAACTAAGCCTCAGAGCGGGAGTTTTCTTGTACAAAGAATTAGCAA	\\	&	TTTTATTAA	\\
(6,0) Core Strand 114	&	GCAACAGGAAAAACGCATGTAGCATTCCAAAGCAAGCA	\\			
(6,0) Core Strand 115	&	GAGAATATGCCAACATTTAAGACGCTGAGAAGCGTCGCTAAGCTACA	\\	&	A	\\
(6,0) Core Strand 116	&	TAAATAGTCAATAATCAAAGGTAAAGTAATTCTGTCCTTGCACCC	\\			
(6,0) Core Strand 117	&	GTGTACTGGTAATTTACATTTGCCTTTAGCGCAGCGGAGATCTTTTC	\\			
(6,0) Core Strand 118	&	CGGTTTATCAGTTTTCTGTATTTTTGGGATTTAGCCTTTTACCACCG	\\	&	GAA	\\
(6,0) Core Strand 119	&	CAGTACCACTGAGACTGAGCCGCCACCAGAACCGCCTCC	\\			
(6,0) Core Strand 120	&	AGCATCGGAACGAGGGTCTTAAAGATATAAAATTGTATCTCAGAGC	\\			
(6,0) Core Strand 121	&	ATTGCATCAAAAAGATGTGCGTTGGGAAGAAAGGTTGTACGTTGAGA	\\	&	T	\\
(6,0) Core Strand 122	&	GGAGAACATAAAATGTGCAATAAATGCAGATACATAATTTTCCAAAA	\\	&	GGAATTACG	\\
(6,0) Core Strand 123	&	TGCTGTAGAGGTCATTTACCAGACGACGATAAAGGCATA	\\			
(6,0) Core Strand 124	&	CGTAAAACTAGCATGAAAGGCCGAAAGTACGCTGAGTAAGTAAGAGC	\\			
(6,0) Core Strand 125	&	TTCAATTAAATCAGATTTTTAATGGAAACAGTACATAAA	\\			
(6,0) Core Strand 126	&	TTCATTTTCGTAGGAATCTGTGAGTGTTTTTAACCTTGCTTCTG	\\			
(6,0) Core Strand 127	&	TGTGTAGTATTTCAAATACATTTCGCAATTTTTCAATAACC	\\			
(6,0) Core Strand 128	&	AGTCAGACCACAAGGAAAGCGTAAGAACATTCACTGCCCATAGTTAC	\\	&	TGTAGCATAGAAAGG	\\
(6,0) Core Strand 129	&	GGAACCAGTGCTAAACTGCTTTGAATAATAAT	\\			
(6,0) Core Strand 130	&	GGGAGAGCCGGAAACGAACCCATTCAGAACCGATAGCAACGTTGAAA	\\			
(6,0) Core Strand 131	&	CAGGATATAGCTGAAAAGGTGGCATTTCATTTCATTATGA	\\			
(6,0) Core Strand 132	&	GTTGGGCGAGGGTGAGCCATTAGCGCAAGGATAAAAATTTTTAGAA	\\			
(6,0) Core Strand 133	&	AACACTATCATTTGAATTACCTTATAATATACCCTCGAA	\\			
(6,0) Core Strand 134	&	CCGCACAGGCGGCCTTTACCGCCATTCCTTATAAACCAATGGCTTAT	\\	&	C	\\
(6,0) Core Strand 135	&	CGGGTCACCGTCACCCGACAATGACAACAATTTTCCATCGCCTCAGA	\\	&	CGACTCGTCAT	\\
(6,0) Core Strand 136	&	GGTAATGGTTTTGTAAAGGTAGTTATTTTAAGGCCGCTTTTGCGGGA	\\	&	TTGTTGCCC	\\
(6,0) Core Strand 137	&	GCTTTAAACAGTTCAGAGAGTCTGGAGCAATAAATCA	\\			
(6,0) Core Strand 138	&	TTCATAACGAAGTTTCAATTGCTATGTACCCCGGTTGATATAAGCA	\\			
(6,0) Core Strand 139	&	AGAGCCAGCAAAATCAGAGCCATTGAGTGAGCAGTGTAAA	\\			
(6,0) Core Strand 140	&	CGTATTGGAACGCGCGTGAAATTGTTATCCGCTCACAATTTTTTCCA	\\	&	CACAACATAC	\\
(6,0) Core Strand 141	&	TCATGTTTGATGGTGGTTTGTCACAATCAATACAAAAGGGGTACCGA	\\	&	TCCTGTG	\\
(6,0) Core Strand 142	&	AACCCTCATCAGATGAATATACAGATTTTCAGATCGGCCTTGCCTGA	\\	&	G	\\
(6,0) Core Strand 143	&	CTCAATCGAACCGTTGTAGCAATTTTTTCTTTGATTA	\\			
(6,0) Core Strand 144	&	AAACCAAAATTTAAATATGCAACTGAGACAGTATTCAAAGTTGTGTA	\\	&	AAGAGAC	\\
(6,0) Core Strand 145	&	AAGAGTAAAAGCGCCAGGGCGATGCAGAAACAGCGGAT	\\			
(6,0) Core Strand 146	&	ATCTCCAAAAAAAAAAGGGGCGCGCAGAGCCATCCCGGAA	\\			
(6,0) Core Strand 147	&	GCTTTCGAGGTGAATTGTACCGTTTTTTCAGCCCAATAG	\\			
(6,0) Core Strand 148	&	TGTAAAACGACGGCCATTTGTGAGGCAAGGCGTTTACCAG	\\			
(6,0) Core Strand 149	&	TTAATTAATTTTCCCTTAGAATCTAGCGATAGACAATAATTCGAGCC	\\	&	CTGAACAA	\\
(6,0) Core Strand 150	&	AAGCGCATTTTGTCTCTGAATTTACCGCTGAGGCT	\\			
(6,0) Core Strand 151	&	AGAGGAAGAGAAAGATTCACCCTCAGAGCCACCGGAATAGTAGCGGG	\\	&	GCTACAG	\\
(6,0) Core Strand 152	&	AATTCTTATCATCTTCTGACCTATTTTTGTTTAACGTCAAAAATGTT	\\	&	TTTAGCAGCC	\\
(6,0) Core Strand 153	&	ACCAGACCCATAAATCAAAAATCTGAGAGATCTACAAAGGCTATCAG	\\	&	TTTTTTGCCT	\\
(6,0) Core Strand 154	&	ACAGTAGAAAACTTTTTCAAATTTTACAGA	\\			
(6,0) Core Strand 155	&	CCCTGCCTTTTTATTTCGGAACCAGAATGGA	\\			
(6,0) Core Strand 156	&	TTGCTATTAGACGACGCTTAGAGTAATTTAGGCAGAGGCAAAGTT	\\			
(6,0) Core Strand 157	&	TTAAAGCCTATTATTCCGCCAGTTTTCATTGACACAGTTAATGCC	\\			
(6,0) Core Strand 158	&	GAGCCTTTGTATAGCCCACCCTCACCTCAAGAGAAGGATTAGGATTA	\\			
(6,0) Core Strand 159	&	TTAGACTCAGAGGGCGAGCTTCAAAGCGA	\\			
(6,0) Core Strand 160	&	ATATTTTTTTTTAATTCCATTTTTAAAGCCAACGCTCA	\\			
(6,0) Core Strand 161	&	GAAATTTTAGAATGACGGAAGCAATTTTCCAACAGGTCAGGATTA	\\			
(6,0) Core Strand 162	&	TAGTTTGACCAATTCTTGCAATGCGTGTCTGCCTCGTTTTTGCGGAT	\\	&	GGCTTA	\\
(6,0) Core Strand 163	&	GTTGGGTTACCTTTCATATGCGTTATACA	\\			
(6,0) Core Strand 164	&	AGCGTCATCCGTATAAAGGAGGTTGGCATTTT	\\			
(6,0) Core Strand 165	&	ACCCTGACTTTTAATTGGTAATAGAACGGAAC	\\			
(6,0) Core Strand 166	&	CCTCAAATGAGAGTACGAGGCTTTTGCAATTTTAGAAGTTTTGC	\\			
(6,0) Core Strand 167	&	GAGATAAACACCGGAAAATTACATTTAACAAT	\\			
(6,0) Core Strand 168	&	AACGCGAGGGCTTAATTATCAAAATCATAGGTCTTTTTAGAGAC	\\			
(6,0) Core Strand 169	&	ACAGTGCACATGGCTTTTCATCGAGGCAGGTCAGACGATTGTTTTGC	\\	&	CTTGATATTCACAAAC	\\
(6,0) Core Strand 170	&	ATTTTTGTACAAGAGAATGATATTGGAATCGTCATAAAT	\\			
(6,0) Core Strand 171	&	GCGTTAAATAAGACTTATTTTCAT	\\			
(6,0) Core Strand 172	&	AAAGCCTGATACCGACATGATGAACGGCTTAG	\\			
(6,0) Core Strand 173	&	TATATAACTTTTATATGTAAATGCTGATGC	\\			
(6,0) Core Strand 174	&	TGGATAATAACGGAACTGCGCGGCGGCGTTTTGGCCGTTCCCTGCAC	\\	&	ACGCAT	\\
(6,0) Core Strand 175	&	CCACCACCAAACGTCGAGAGGGTTCAGCTTGA	\\			
(6,0) Core Strand 176	&	AGGCTTTGAGGACTAAATACCAGT	\\			
(6,0) Core Strand 177	&	GGATAGCGTCCTTTTATACTGCCAACCGTTCTTTTAGCTGATAAATT	\\	&	AATGCC	\\
(6,0) Core Strand 178	&	GAATTTTTAGAGCGTAATGCGTATCCCAATCCACAC	\\			
(6,0) Core Strand 179	&	AGGGAGCCACATAAAACCAGTTACAAAATAAACATTTTCCATATTAT	\\	&	T	\\
(6,0) Core Strand 180	&	GAAATAGCAATAGCTGCAGTATGCCGGTGCC	\\			
(6,0) Core Strand 181	&	AAGTTTCCATTAAACGGACGGGCAACAGCTTA	\\			
(6,0) Core Strand 182	&	GACGGGGATTTTCGGCGAACGTGGCGAGAGGGCTTTTCGTACTATGG	\\			
(6,0) Core Strand 183	&	TAGGAGCACTAACAACTGAGTAACGCCGCGCT	\\			
(6,0) Core Strand 184	&	TAAAACAGAACAATTCTATTAAATTTGCTTTGACGAGCA	\\			


